Electrodynamic properties of graphene and their technological applications

Graphene is a novel two-dimensional material with fascinating electrodynamic properties like the ability to support collective electron oscillations (plasmons) accompanied by tight confinement of electromagnetic fields. Our goal is to explore light-matter interaction in graphene in the context of plasmonics and other technological applications but also to use graphene as a platform for studying many body physics like the interaction between plasmons, phonons and other elementary excitations. Plasmons and plasmon-phonon interaction are analyzed within the self-consistent linear response approximation. We demonstrate that electron-phonon interaction leads to large plasmon damping when plasmon energy exceeds that of the optical phonon but also a peculiar mixing of plasmon and optical phonon polarizations. Plasmon-phonon coupling is strongest when these two excitations have similar energy and momentum. We also analyze properties of transverse electric plasmons in bilayer graphene. Finally we show that thermally excited plasmons strongly mediate and enhance the near field radiation transfer between two closely separated graphene sheets. We also demonstrate that graphene can be used as a thermal emitter in the near field thermophotovoltaics leading to large efficiencies and power densities. Near field heat transfer is analyzed withing the framework of fluctuational electrodynamics.

==> chap7.tex <==
\chapter{Near field thermo-photo-voltaics using graphene as a thermal emitter} \label{chap:chap7}


Here we show that graphene can be used as a thermal emitter in the near field thermo-photo-voltaic (TPV) system resulting in high efficiencies and power densities. The near field heat transfer is mediated by thermally excited plasmon modes in graphene similarly to the situation in the last subsection. 

The system we analyze consists of a hot graphene emitter at a temperature $T_1$ and a photo-voltaic (PV) cell held at room temperature $T_2=300$K and distance $D$ away from graphene. It is interesting to note that the expression for the near field heat transfer between graphene and a PV cell is given by the same expression (\ref{H_nf}) for the graphene to graphene heat transfer:
%
\begin{equation}
H_{nf}=\frac{1}{(2\pi)^3} 
\int_{0}^{\infty} d\omega 
\left[ 
\frac{\hbar\omega}{e^{\beta_1\hbar\omega}-1} -
\frac{\hbar\omega}{e^{\beta_2\hbar\omega}-1}
\right]
\int_{\omega/c}^{\infty} 2\pi q dq
h_{nf}^p (q,\omega)
\label{H_nf2}
\end{equation}
%
\begin{equation}
h^p_{nf}({\bf q},\omega)  \equiv 
\frac{\Im r_1^p \Im r_2^p e^{-2q D}}
{|1 - r_1^p r_2^p e^{-2q D}|^2}
\label{h_nf2}
\end{equation}
%
Here we have neglected the contribution from $s$ polarization, and assumed $\gamma=\sqrt{\omega^2/c^2-q^2}\approx iq$ since the near field heat transfer is mediated by graphene plasmon modes in the non-retareded regime ($q>>\omega/c$). To model graphene we use $q$-independent conductivity $\sigma(\omega)$ from equation (\ref{eq:cond}) as before, and the reflection coefficient is given by equation (\ref{r_p}) which we write again for the sake of clearance:
%
\begin{equation}
r_1^p(q,\omega)=\frac{ \frac{i q \sigma(\omega)}{2\epsilon_0\omega} }
         { 1+ \frac{i q \sigma(\omega)}{2\epsilon_0\omega}}
\label{r_graphene}
\end{equation}
%
Above hot graphene emitter we now have PV cell which we model as a simple direct band-gap semiconductor with parameters:
%
\begin{align}
    \epsilon_2(\omega) = \left(n+i\frac{\alpha}{2k_0}\right)^2
    \quad \mathrm{where} \quad \alpha(\omega) = \left\{ \begin{array}{ll} 0
    &, \omega < \omega_g \\ \alpha_0 \sqrt{\frac{\omega-\omega_g}{\omega_g}}
    &, \omega > \omega_g \end{array} \right. 
\label{eq:eps2}
\end{align}
%
Here $n$ is the refractive index, $k_0=2\pi/\lambda=c/\omega$ is the photon wavelength in vaccum, and $\omega_g$ is the bandgap frequency.
Speciffically we will discuss the case of indium antimonide (InSb)     
with parameters $\omega_g=0.17eV$ and $\alpha_0 \approx 0.7 \times 10^4 cm^{-1}$ 
(at room temperature \cite{Gobeli1960}). Finally the reflection coefficient of the PV cell, in the non-retarded regime ($q>>\omega/c$), is simply given by \cite{Jackson}:
%
\begin{equation}
r_2^p(\omega)=\frac{\epsilon_2(\omega)-1}{\epsilon_2(\omega)+1}
\label{r_PV}
\end{equation}
%
When the PV cell is biased at a voltage \footnote{In
general, the optimal voltage $V_o$ depends on other parameters in the
system. We avoid the full optimization procedure, and, motivated by the
observed dependence of efficiency on $V_o$, choose a voltage slightly
below the limit $V_o^{max}=\omega_g(1-T_2/T_1)$.} $V_o$, we can express the total radiative power exchange as
\cite{Celanovic2004}: 
%
\begin{equation}
P_{rad}=\frac{1}{(2\pi)^3} 
\int_{0}^{\infty} d\omega 
\left[ 
\frac{\hbar\omega}{e^{\beta_1\hbar\omega}-1} -
\frac{\hbar\omega}{e^{\beta_2(\hbar\omega-V_o)}-1}
\right]
\int_{\omega/c}^{\infty} 2\pi q dq
h_{nf}^p (q,\omega)
\label{P_rad}
\end{equation}
%
On the other hand we can also write the total photon flux into the PV cell as:
%
\begin{equation}
j_{ph}=\frac{1}{(2\pi)^3} 
\int_{0}^{\infty} d\omega 
\left[ 
\frac{1}{e^{\beta_1\hbar\omega}-1} -
\frac{1}{e^{\beta_2(\hbar\omega-V_o)}-1}
\right]
\int_{\omega/c}^{\infty} 2\pi q dq
h_{nf}^p (q,\omega)
\label{j_ph}
\end{equation}
%
In the case of ideal PV cell, also know as Shockley-Quiesser limit \cite{Shockley}, the only limiting factor is the radiative recombination of charge carriers so the electron current is simply: $j_e=e j_{ph}$. Then the electrical power generated in the PV cell is $P_{PV}=j_e V_o$, and efficiency of  device is:
%
\begin{equation}
\eta_{TPV} = 
\frac{P_{PV}}{P_{rad}} = 
\frac{e j_{ph}V_o}{P_{rad}}
\label{efficiency}
\end{equation}
%
Let us now choose the graphene's chemical potential to be $\mu=0.2eV$, and that the PV cell is held at room temperature $T_2=300$K and distance $D=10$nm away from the graphene sheet. Then for the case of graphene's temperature $T_1=600(1200)$K and biased voltage $V_o=0.08(0.12)$V, the output power density of our TPV device is $P_{PV}/A=4.4(110)W/cm^2$ with an efficiency of $\eta=31(42)\%$. We note that these are remarkably high power densities considering that our thermal emitter is only one atom thick. To get a better sense of the scales involved we can compare the far field radiative power exchange $P_{rad}^{BB}$ between two black bodies held at temperatures $T_1$ and $T_2$ but involving only the photons of energies above the PV band gap, and the near field radiative power exchange $P_{rad}^{gPV}$ between graphene and a PV cell held at these temperatures. For the temperatures $T_1=600(1200$)K and $T_2=300$K one obtains $P_{rad}^{gPV}/P_{rad}^{BB}=45(27)$ times increase over the black body case. Further on, note that the near field heat transfer is particularly convenient since the energy is transfered by the evanescent modes and the photons with an energy below the band gap, that are not absorbed by the PV cell, simply return to the graphene emitter as heat, unlike the far field case where they are lost in the form of propagating waves. This results in the high efficiencies $\eta=31(42)\%$, however note that these numbers are still below the Carnot limit $\eta=50(75)\%$  for temperatures $T_1=600(1200$)K and $T_2=300$K. The reson for this is the broad band plasmon spectrum contributing to the heat transfer with the high energy photons ($E>\hbar\omega_g$) wasting the energy difference ($\Delta E=E-\hbar\omega_g$) on the thermalization losses heating up the system. To achieve even higher efficiencies one would need to tailor the emitter properties so that it selectively radiates only in the small interval around the band gap of the PV cell. One way to do this would be to use surface plamons at metal-dielectric surface, since they have very large density of states around the surface plasmon resonance; see figure \ref{Figure1_c3} b, and compare it to broad band spectrum of graphene plasmon mode from figure \ref{Figure2_c3} d. However, the problem with metals is that surface plasmon resonance usually falls in the visible/ultraviolet regime which is impossible to excite thermally. Alternativelly one could use highly doped semiconductors like Indium-Tin-Oxide \cite{ITO} which has a resonance in the infra-red \cite{ITO_plasmonic}, however due to high doping level there is a lot of electron-impurity scattering and high losses result in reduced efficiencies. In that regards graphene TPV system shows large promise for a new temperature range ($600-1200$K) solid state energy conversion, where conventional thermoelectrics can not operate due to high temperatures and far field TPV schemes suffer from low efficiency and power density.



